Fair Federated Data Clustering through Personalization: Bridging the Gap between Diverse Data Distributions

The rapid growth of data from edge devices has catalyzed the performance of machine learning algorithms. However, the data generated resides at client devices thus there are majorly two challenge faced by traditional machine learning paradigms - centralization of data for training and secondly for most the generated data the class labels are missing and there is very poor incentives to clients to manually label their data owing to high cost and lack of expertise. To overcome these issues, there have been initial attempts to handle unlabelled data in a privacy preserving distributed manner using unsupervised federated data clustering. The goal is partition the data available on clients into $k$ partitions (called clusters) without actual exchange of data. Most of the existing algorithms are highly dependent on data distribution patterns across clients or are computationally expensive. Furthermore, due to presence of skewed nature of data across clients in most of practical scenarios existing models might result in clients suffering high clustering cost making them reluctant to participate in federated process. To this, we are first to introduce the idea of personalization in federated clustering. The goal is achieve balance between achieving lower clustering cost and at same time achieving uniform cost across clients. We propose p-FClus that addresses these goal in a single round of communication between server and clients. We validate the efficacy of p-FClus against variety of federated datasets showcasing it's data independence nature, applicability to any finite $\ell$-norm, while simultaneously achieving lower cost and variance.

==> algo.tex <==
\section{\ouralgo: personalized Federated Clustering}
% \vspace{100pt}
\ouralgo\ begins with each client $z \in [Z]$ executing the $k$-means algorithm locally on their respective datasets $X^{(z)}$, producing individual sets of local centers $C^{(z)}$ = $\{C^{(z)}_1, C^{(z)}_2, \ldots, C^{(z)}_k\}$. Subsequently, these local centers are transmitted to the server for aggregation.
\\
Upon reception, the server employs the Llyod $k$-means clustering on these local centers, thereby generating a set of global centers $G$ = $\{G_1, G_2, \ldots, G_k\}$. This consolidated set is then disseminated back to the clients.
\\
Each client then applies personalization equation (reference) to generate their own unique set of personalized centers $G^{(z)}$ = $\{G^{(z)}_1, G^{(z)}_2, \ldots, G^{(z)}_k\}$. The complete algorithm for \ouralgo\ is described in Algorithm 1 (Reference)

\begin{algorithm}[ht!]
\caption{\ouralgo: {Personalized Federated Clustering } }
\label{algo:csca}
\textbf{Input}: Federated set of datapoints $X$, number of clusters $k$, number of clients $z$ where $X^{(z)}$ refers to the datapoints of $z^{th}$ client \\  %$\alpha$ (using $\Gam$ in Equation \ref{eqn:AlphaDefine})\\
\textbf{Output}:Personalized centers of each client %with centers $\{c_j\}_{j=1}^\ell$ where $\ell \ge k$, and assignment function $\hat{\phi}$

\textbf{Client initially executes: }
\begin{algorithmic}[1] %[1] enables line numbers

\STATE Each client $z \in [Z]$, applies $k$-means clustering with local data $X^{(z)}$ and $k$ to find local cluster centers $C^{(z)}$.
\\
\STATE All clients $z \in [Z]$ share these center sets $C^{(z)}$ with server.\\

\end{algorithmic}
\textbf{Server executes: }
\begin{algorithmic}[1] %[1] enables line numbers
\STATE  Server receives set of centers $C^{(z)}$ from all devices $z \in [Z]$, to construct $S$ = $C^{(1)}\cup C^{(2)}\ldots \cup C^{(z)}$ \\

%\STATE  Compute optimal cost $w^*$ $\gets$ costCapacitatedOffline \\%\min_{x,x' \in C} || x-x'||^2/2$\\
       
\STATE Server applies Llyod $k$-means clustering on set $S$, to find $k$ global centers $G$ = $\{G_1, G_2, \ldots, G_k\}$\\
\STATE Server sends back global centers $G$ to all clients $z \in [Z]$ for personalization. \\

\end{algorithmic}
\textbf{Client personalizes: }
\begin{algorithmic}[1] %[1] enables line numbers

\STATE Each client $z \in [Z]$ runs the following: \\
\STATE $count$[] = 0 \\
\STATE $\lambda$ = 0.01
\FOR{10 iterations}
\FOR{a datapoint $x \in X^{(z)}$}
    \STATE Calculate the closest local center $C'_k$ and closest global center $G'_k$ 
    \STATE $count[G'_k] \mathrel{+}= 1$ 
    \STATE $\eta = \text{Learning Rate} = \frac{1}{\text{count}[G'_k]}$ \\
    \STATE $G'_k =  G'_k - \eta\left((x - G'_k) + 2\lambda (C'_k -G'_k)\right)$ 
\ENDFOR
\ENDFOR
\RETURN  Personalized centers of each client
\end{algorithmic}
\end{algorithm}

%Presenting the personalisation equation
Given a point x, let $G_i$ represents the nearest global center to point x, $C_j$ represents the nearest local center to point x then,

\[ F_x = \frac{1}{2} (x - G_i)^2 + \lambda (G_i - C_j)^2 \]
\[\frac{\partial F_x}{\partial G_i} = x - G_i + 2 \lambda (G_i - C_j)\]
\[ G_i = G_i + \eta\frac{\partial F_x}{\partial G_i} \]
\[ G_i = G_i + \eta [x - G_i + 2\lambda(G_i - C_j)] \]
where $\eta = \frac{1}{\text{count}[G_i]}$ 
\\
\\
\textbf{Lemma 1 } Converges.


==> experi_tarushi_tsering.tex <==
\section{Experimental Analysis}
In this section, we now validate the efficacy of our proposed approach on synthetic and \emph{benchmarking} real-world datasets against different state-of-the-art (\sota) methods.  The datasets used in the study are:
\begin{itemize}
    \item \textbf{Synthetic dataset}:  
    \item \textbf{Adult:} The 1994 census dataset contains 32,562 records of individuals. We evaluate performance on five attributes as a feature set: age, fnlwgt, education\_num, capital\_gain, and hours\_per\_week. These attributes are popular in clustering literature \cite{chierichetti2018fair,ziko2019variational,backurs2019scalable,bera2019fair}. The dataset is publicly available \cite{AdultDataset}. 
    \item \textbf{Bank:} A Portuguese bank marketing dataset of 41,108 records, with each record containing information on the customer's details. We use age, duration, campaign, cons.price.idx, euribor3m, nr.employed as a feature set consistent with clustering literature \cite{chierichetti2018fair,ziko2019variational,backurs2019scalable,bera2019fair}. The dataset is publicly available \cite{BankDataset}.
    \item \textbf{Diabetic:}
    \item \textbf{FMNIST:} It consists of 70,000 images covering ten classes of fashion items at a resolution of 28 × 28, which includes 60,000 training images and 10,000 test images. We only use the training images in the experiments. The dataset is publicly available \cite{xiao2017fashion}.
    \item \textbf{WISDM:} It is a time series dataset consisting of 1,098,207 records of the speed of 36 individuals(total clients) across 3 axis:x,y and z at various timestamp, when doing one among the 6 activites: Walking, Jogging, Upstairs, Downstairs, Sitting and Standing(total clusters). The dataset is obtained from \cite{kwapisz2011activity}
    \item \textbf{Celeba:} It is an image dataset containing 202,599 number of face images of various celebrities with 40 attribute labels each. The preprocessed version publicly available at kaggle\footnote{https://www.kaggle.com/datasets/jessicali9530/celeba-dataset} is used. The original dataset is publicly available \cite{liu2015faceattributes}
    \item \textbf{FEMNIST:} Federated EMNIST is a realistic FL image dataset where the data points are the handwritten digits or letters ranging from 0 to 9 from a specific writer. The experiments were performed on 100 clients. The orginal dataset was obtained from \cite{caldas2018leaf}. Thoda doubt isme.
\end{itemize}
\noindent \textbf{Experimental Setup}:  All experiments are executed on i$5$ $8^{th}$ generation processor, $8$GB RAM and Windows $10$  with Python $3.8$.  We report the mean of  performance  across five independent runs with different seed values from the set $\{0, 100, \ldots, 1200\}$.We examine two different data distribution regimes, namely homogeneous and heterogeneous described in Section below. We limit $k_z$ = $k\ \forall z\in[Z]$ for experimental study in homogenous setting. To distribute data points among clients in a heterogeneous setting, we randomly allocate each client device with data points from exactly $k_z$ distributions i.e, a heterogeneity of $2$ implies each client has points exactly from $2$ of $k$ distributions where $k$ is the target number of clusters.

\noindent \textbf{Baselines:} We evaluate the performance of our proposed algorithm against following: 
\begin{itemize}
    \item \textbf{Centralized $k$-means} (\textbf{C$k$means}): The centralized variation of famous Llyod heuristic also simply known as $k$-means \cite{lloyd1982least}.
    \item \textbf{$k$-FED}:  The method assumes the knowledge of $k_z$ on each client device. Each client utilizes this information and executes the Llyod heuristic to obtain local clustering. These are then accumulated over all clients at the server to compute global $k$-clustering. 
    \item \textbf{$MFC$}: After the initial handshake between the client and server as in $k$-FED, they engage in multiple rounds of communication where Clients use the global centers to update their local assignment functions by re-assigning each data point to the nearest center.  The local cluster centers are updated by taking the mean of points assigned to each center.  The client sends the local cluster center back with the maximum clustering cost on local data. Conversely, when the server receives the maximum cost centers, it recalculates the global centers by using Lloyd's $k$-means on the previous global centers and local cluster centers sent from all clients. After finding the updated global centers, they are returned to the clients. This iterative process is repeated for a few rounds until convergence is reached.
\end{itemize}
\noindent \textbf{Dataset Description:}

\subsection{Synthetic Datasets:} 
    \subsubsection{Equal data per client:}
    In this we further considered 2 types of settings- Homogeneous setting where each client got data from all gaussians(20) and Heterogeneous setting where each client got data from varying gaussians which were mainly 3,5,7,10,12,15 and 18. Further we considered three types of overlaps between these gaussians: little,lot and no overlap.
    
    \subsubsection{Unequal data per client:}
    Here also all parameters were kept same as above but only the number of datapoints per client were different.
    
\subsection{Real World Datasets:}
    \subsubsection{Description}
    There are two kinds of real world datasets we have considered: first, those datasets which are not federated. That is, the data is not divided among clients naturally. These datasets are: Adult, Bank and Diabetic. For these type of datasets, we tried dividing the data creating different federated scenarios which is explained more clearly in below subsections.
    \newline Secondly, we have considered federated datasets which means they already have fixed homogeneity and are already divided across fixed number of clients. These datasets are: WISDM, CELEBA FEMNIST and FMNIST.
    \subsubsection{Equal data per client}
    In this type of data setting, all data points of the dataset is equally distributed among all the clients. Keeping the data points across the clients equal, there is another variation on homogeneity, that is, number of gaussians each client is getting their data from. We have total of 10 gaussians and have considered homogeneity 2, 5, 7 and 10 as below:
 \begin{itemize}
  \item homogeneity 2(hetrogenous)
  \newline Each client gets all its data from only 2 of the gaussians
  \item homogeneity 5(hetrogenous)
  \newline Each client gets all its data from only 5 of the gaussians
  \item homogeneity 7(hetrogenous)
  \newline Each client gets all its data from only 7 of the gaussians
  \item homogeneity 10(homogenous)
  \newline Each client gets its data from all of the gaussians
 \end{itemize}
Below is the detailed description of adult, bank and diabetic dataset settings.
\begin{itemize}
    \item Adult Dataset
    \newline Total number of data-points: 32561
    \newline Total classes: 10
    \newline For 100 clients setting, each client have 325 or 326 data points.
    \newline For 1000 clients setting, each client have 32 or 33 data points.
    \item Bank Dataset
    \newline Total number of data-points: 41108
    \newline Total classes: 10
    \newline For 100 clients setting, each client have 411 or 412 data points.
    \newline For 1000 clients setting, each client have 41 or 42 data points.
    \item Diabetic Dataset
    \newline Total number of data-points: 101763
    \newline Total classes: 10
    \newline For 100 clients setting, each client have 1016 or 1017 data points.
    \newline For 1000 clients setting, each client have 100 or 101 data points.
\end{itemize}

\subsubsection{Unequal data per client}
In this type of data setting, different clients have different number of data points. We have tried making a very distributed setting where few clients have data points upto 2000, 4000, 6000 etc and on the other hand few clients have only 10 data points.
And for the rest, they have their data size ranging in between these numbers.We tried increasing the data size *****. Keeping the data points across the clients unequal, we have also varied the heterogeneity of the dataset as done earlier as follows:
 \begin{itemize}
  \item homogeneity 2(hetrogenous)
  \newline Each client gets all its data from only 2 of the gaussians
  \item homogeneity 5(hetrogenous)
  \newline Each client gets all its data from only 5 of the gaussians
  \item homogeneity 7(hetrogenous)
  \newline Each client gets all its data from only 7 of the gaussians
  \item homogeneity 10(homogenous)
  \newline Each client gets its data from all of the gaussians
 \end{itemize}
Below is the detailed description of adult, bank and diabetic dataset settings.
\begin{itemize}
    \item Adult Dataset
    \newline Total number of data-points: 32561
    \newline Total classes: 10
    \newline For 100 clients setting, they have data size ranging from 10 to 4000s.
    \newline For 1000 clients setting, they have data size ranging from 10 to 2000 or 3000. 
    \item Bank Dataset
    \newline Total number of data-points: 41108
    \newline Total classes: 10
    \newline For 100 clients setting, they have data size ranging from 10 to 5000s.
    \newline For 1000 clients setting, they have data size ranging from 10 to 3000 or 4000. 
    \item Diabetic Dataset
    \newline Total number of data-points: 101763
    \newline Total classes: 10
    \newline For 100 clients setting, they have data size ranging from 10 to 5000 or 6000s.
    \newline For 1000 clients setting, they have data size ranging from 10 to 3000 or 4000.
\end{itemize}
\subsubsection{Other setings}
For the rest of the datasets, WISDM, FEMNIST, FMNIST and CELEBA, their data was already in a federated setting. This implies that a data point already belongs to a gaussian and was assigned to a client as well. This makes the dataset to naturally have a fix distribution, homogeneity and number of clients. Hence we have used these datasets as they were for our experiments.
\newline
\newline

\noindent \textbf{Graphs and Results}
\subsection{Adult}
\subsubsection{Equal}
\begin{figure*}[ht!]
\centering
\begin{tabular}{@{}c@{}c@{}c@{}c@{}}
\includegraphics[width=0.35\textwidth]{images/adult_Hetero_equal_100_clients_mean_cost.png}&\includegraphics[width=0.33\textwidth]{images/adult_Hetero_equal_100_clients_std_dev.png}&\includegraphics[width=0.33\textwidth]{images/adult_Hetero_equal_100_clients_max_cost.png}\\
\includegraphics[width=0.35\textwidth]{images/adult_Hetero_equal_1000_clients_mean_cost.png}&\includegraphics[width=0.33\textwidth]{images/adult_Hetero_equal_1000_clients_std_dev.png}&\includegraphics[width=0.33\textwidth]{images/adult_Hetero_equal_1000_clients_max_cost.png} \\
\end{tabular}
  \caption{The graphs in the first row shows the mean clustering cost per point, standard deviation per point and maximum clustering cost per point respectively for data setting of 100 clients and each client having equal number of data points. The graphs in the second row shows the same but for 1000 clients having equal number of data points.}
    \label{fig:costVariation}
\end{figure*}

Results: Ditto mean cost is significantly  less than others, even on increasing number of clients.
\newline
Fairness metric (std dev.) is stable for Ditto and lies within a fixed range even on varying homogeneity.
\newline
Max. cost is higher for k-FED and MFC but max. Cost for ditto increases as homogeneity increases as we have fixed equal data across clients and on increasing homogeneity (k’) number of data points from each clusters reduces so the k >= k’ results in slightly higher max costs. Earlier, for say two clusters we were giving three centers so max cost was less.   
\newline
Std dev. of k-FED and MFC is higher at smaller homogeneity as intrinsically these algo’s do not provide personalization whereas fine tuning on local data helps improvise centers according to current dynamic nature of local data. Std dev. of k-FED and MFC drops only below Ditto at high homogeneity as then these algo’s are able to capture good estimates of center due to presence of centers from almost all gaussians at each client whereas ditto is able to maintain good estimate of centers at low homogeneity as well thus, ensuring  a consistent methodology with more easy real-world implementation as one need not worry about the level of present homogeneity. 
\newline Thus Ditto is better in this setting !!
\newline
\newline
\subsubsection{Unequal}
\begin{figure*}[ht!]
\centering
\begin{tabular}{@{}c@{}c@{}c@{}c@{}}
\includegraphics[width=0.35\textwidth]{images/adult_Hetero_unequal_100_clients_mean_cost.png}&\includegraphics[width=0.33\textwidth]{images/adult_Hetero_unequal_100_clients_std_dev.png}&\includegraphics[width=0.33\textwidth]{images/adult_Hetero_unequal_100_clients_max_cost.png}\\
\includegraphics[width=0.35\textwidth]{images/adult_Hetero_unequal_500_clients_mean_cost.png}&\includegraphics[width=0.33\textwidth]{images/adult_Hetero_unequal_500_clients_std_dev.png}&\includegraphics[width=0.33\textwidth]{images/adult_Hetero_unequal_500_clients_max_cost.png} \\
\end{tabular}
  \caption{The graphs in the first row shows the mean clustering cost per point, standard deviation per point and maximum clustering cost per point respectively for data setting of 100 clients and all client having unequal number of data points. The graphs in the second row shows the same but for 500 clients having unequal number of data points.}
    \label{fig:costVariation}
\end{figure*}

Results: Ditto mean cost is significantly less than others, even on increasing number of clients.
\newline
Fairness metric (std dev.) is stable for Ditto and lies within a fixed range even on varying homogeneity.

Max. cost is higher for k-FED and MFC but max. Cost for ditto increases as homogeneity increases on similar reasons as in equal data case. 

(100 Clients): Std dev. of k-FED and MFC is higher at smaller homogeneity with high deviation over independent runs but Std dev. of k-FED and MFC drops only below Ditto as homogeneity increases as then due to presence of unequal data on clients, these algo’s are able to capture estimation of centers, but still have higher deviation over independent runs. On contrary, Ditto has fairness level maintained across varying homogeneity showing that algorithm is not dependent on how data is distributed among clients and works well for across different cases. Further, in case of 100 clients MFC and k-FED started performing well on homogeneity beyond 3 but in case of 500 clients it dropped sharply, showcasing that the MFC and k-FED approach are not reliable in terms of fairness whereas Ditto fairness always decrease or remain at a level on increasing homogeneity. 
\newline Thus Ditto is better in this setting !!

\subsection{Bank}
\subsubsection{Equal}
\begin{figure*}[ht!]
\centering
\begin{tabular}{@{}c@{}c@{}c@{}c@{}}
\includegraphics[width=0.35\textwidth]{images/bank_Hetero_equal_100_clients_mean_cost.png}&\includegraphics[width=0.33\textwidth]{images/bank_Hetero_equal_100_clients_std_dev.png}&\includegraphics[width=0.33\textwidth]{images/bank_Hetero_equal_100_clients_max_cost.png}\\
\includegraphics[width=0.35\textwidth]{images/bank_Hetero_equal_1000_clients_mean_cost.png}&\includegraphics[width=0.33\textwidth]{images/bank_Hetero_equal_1000_clients_std_dev.png}&\includegraphics[width=0.33\textwidth]{images/bank_Hetero_equal_1000_clients_max_cost.png} \\
\end{tabular}
  \caption{The graphs in the first row shows the mean clustering cost per point, standard deviation per point and maximum clustering cost per point respectively for data setting of 100 clients and each client having equal number of data points for bank dataset. The graphs in the second row shows the same but for 1000 clients having equal number of data points.}
    \label{fig:costVariation}
\end{figure*}

Results: Ditto mean cost is significantly  less than others, even on increasing number of clients.
\newline Unlike adult dataset, std dev of MFC/k-FED is always higher than ditto and does not fall below ditto after certain homo. 
\newline Thus Ditto is much better in this setting !!
\newline
\newline
\subsubsection{Unequal}
\begin{figure*}[ht!]
\centering
\begin{tabular}{@{}c@{}c@{}c@{}c@{}}
\includegraphics[width=0.35\textwidth]{images/bank_Hetero_unequal_100_clients_mean_cost.png}&\includegraphics[width=0.33\textwidth]{images/bank_Hetero_unequal_100_clients_std_dev.png}&\includegraphics[width=0.33\textwidth]{images/bank_Hetero_unequal_100_clients_max_cost.png}\\
\includegraphics[width=0.35\textwidth]{images/bank_Hetero_unequal_500_clients_mean_cost.png}&\includegraphics[width=0.33\textwidth]{images/bank_Hetero_unequal_500_clients_std_dev.png}&\includegraphics[width=0.33\textwidth]{images/bank_Hetero_unequal_500_clients_max_cost.png} \\
\end{tabular}
  \caption{The graphs in the first row shows the mean clustering cost per point, standard deviation per point and maximum clustering cost per point respectively for data setting of 100 clients and all client having unequal number of data points for bank dataset. The graphs in the second row shows the same but for 500 clients having unequal number of data points.}
    \label{fig:costVariation}
\end{figure*}
Results: Again, coming to std dev, as in adult dataset, here also MFC and k-FED has quite different patterns (arbitrary trend) as homo and number of clients changes. Whereas Ditto maintains  a upper threshold on std dev (fairness level) and always remain below that, whereas other algo’s are sensitive to number of clients and homo. 
\newline Thus Ditto remains a better choice !!
\subsection{Diabetic}
\subsubsection{Equal}
\begin{figure*}[ht!]
\centering
\begin{tabular}{@{}c@{}c@{}c@{}c@{}}
\includegraphics[width=0.35\textwidth]{images/diabetic_100c_equal_mean.png}&\includegraphics[width=0.33\textwidth]{images/diabetic_100c_equal_std_dev.png}&\includegraphics[width=0.33\textwidth]{images/diabetic_100c_equal_max_cost.png}\\
\includegraphics[width=0.35\textwidth]{images/diabetic_1000c_equal_mean.png}&\includegraphics[width=0.33\textwidth]{images/diabetic_1000c_equal_std_dev.png}&\includegraphics[width=0.33\textwidth]{images/diabetic_1000c_equal_max_cost.png} \\
\end{tabular}
  \caption{The graphs in the first row shows the mean clustering cost per point, standard deviation per point and maximum clustering cost per point respectively for data setting of 100 clients and each client having equal number of data points for diabetic dataset. The graphs in the second row shows the same but for 1000 clients having equal number of data points.}
    \label{fig:costVariation}
\end{figure*}

Results: Mean cost is lowest for our algorithm in almost all cases.
\newline Max cost in our algorithm is either lower or comparable to other algorithms.
\newline Fairness metric (Std dev.) of K-FED and MFC are higher at smaller homogeneity and drops below Ditto at high homogeneity. i.e. our algorithm is performing better for less homogeneity.
\newline Thus Ditto is having reasonable fairness while having lower cost in this setting.
\newline
\newline
\subsubsection{Unequal}
\begin{figure*}[ht!]
\centering
\begin{tabular}{@{}c@{}c@{}c@{}c@{}}
\includegraphics[width=0.35\textwidth]{images/diabetic_100c_unequal_mean.png}&\includegraphics[width=0.33\textwidth]{images/diabetic_100c_unequal_std_dev.png}&\includegraphics[width=0.33\textwidth]{images/diabetic_100c_unequal_max_cost.png}\\
\includegraphics[width=0.35\textwidth]{images/diabetic_500c_unequal_mean.png}&\includegraphics[width=0.33\textwidth]{images/diabetic_500c_unequal_std_dev.png}&\includegraphics[width=0.33\textwidth]{images/diabetic_500c_unequal_max_cost.png} \\
\end{tabular}
  \caption{The graphs in the first row shows the mean clustering cost per point, standard deviation per point and maximum clustering cost per point respectively for data setting of 100 clients and all client having unequal number of data points for diabetic dataset. The graphs in the second row shows the same but for 500 clients having unequal number of data points.}
    \label{fig:costVariation}
\end{figure*}
Results:
\newline 
\subsection{FMNIST}
\begin{figure*}[ht!]
\centering
\begin{tabular}{@{}c@{}c@{}c@{}c@{}}
\includegraphics[width=0.35\textwidth]{images/fmnist_c500_uniform_mean.png}&\includegraphics[width=0.33\textwidth]{images/fmnist_500c_uniform_std_dev.png}&\includegraphics[width=0.33\textwidth]{images/fmnist_500c_uniform_max_cost.png}\\
\includegraphics[width=0.35\textwidth]{images/fmnist_c1000_uniform_mean.png}&\includegraphics[width=0.33\textwidth]{images/fmnist_1000c_uniform_std_dev.png}&\includegraphics[width=0.33\textwidth]{images/fmnist_1000c_uniform_max_cost.png} \\
\end{tabular}
  \caption{The graphs in the first row shows the mean clustering cost per point, standard deviation per point and maximum clustering cost per point respectively for data setting of 500 clients for FMNIST dataset. The graphs in the second row shows the same but for 1000 clients.}
    \label{fig:costVariation}
\end{figure*}
Results:Mean clustering cost per point is significantly lowest in our algorithm for both 500 and 1000 clients and all homogeneity.
\newline Max clustering cost per point is also least for our algorithm.
\newline Standard deviation is comparable in all three algorithms.
\newline Thus Ditto is better in this setting.
\subsection{WISDM}
\begin{figure*}[ht!]
\centering
\begin{tabular}{@{}c@{}c@{}c@{}c@{}}
\includegraphics[width=0.35\textwidth]{images/wisdm_results.png}\\
\end{tabular}
  \caption{The graph shows mean clustering cost, standard deviation and max clustering cost of WISDM dataset.}
    \label{fig:costVariation}
\end{figure*}
Results: Ditto is better in this setting !!
\newline Scale is 1e13 ?
\subsection{FEMNIST}
\begin{figure*}[ht!]
\centering
\begin{tabular}{@{}c@{}c@{}c@{}c@{}}
\includegraphics[width=0.35\textwidth]{images/pca_femnist_c100_results.png}\\
\end{tabular}
  \caption{The graph shows mean clustering cost, standard deviation and max clustering cost of FEMNIST dataset with 100 clients.}
    \label{fig:costVariation}
\end{figure*}
Results: Ditto is better in this setting !!
\subsection{CELEBA}
need to run the algorithm




==> intro.tex <==
\section{Federated Learning}
Federated Learning (FL), firstly introduced by Google, in 2016, to predict user’s text input within tens of thousands Android devices while keeping data on devices, is an encrypted distributed learning paradigm that enables  resource-constrained edge compute devices, such as mobile phones and IoT devices to train machine learning models collaboratively without centralized data sharing. Specifically, each participant trains a local model on their private data, and only the model updates are exchanged with a central server for aggregation and finally the server sends the model update to the participants to achieve the learning goal. The accuracy of the federated model is an optimal approximation of the accuracy of the ideal model built from centralized data. Federated learning can be divided into horizontal federated learning, vertical federated learning and federated transfer learning according to the distribution of data. Horizontal federated learning is suitable in the case that the user features of the two datasets overlap a lot, but the users overlap little. In horizontal federated learning, it is common for all parties to calculate and upload local gradients so that the central server can aggregate them into a global model.Vertical federated learning is available in the case that the user features of the two datasets overlap little, but the users overlap a lot. In the case that the users and user features of the two datasets both rarely overlap, we can use transfer learning to overcome the lack of data or tags.

Due to the property that data are not exposed to third central server, FL is appropriate for application when data are privacy-sensitive as the emergence of this technology will solve the contradiction between data privacy and data sharing for dispersed devices. These includes cases in health care or mobile devices that data are not available to be aggregated with legal concern. For example, training an AI-based tumour detector requires a large database encompassing the full spectrum of possible anatomies, pathologies, and input data types. Data like this is hard to obtain, because health data is highly sensitive and its usage is tightly regulated. Even if data anonymisation could bypass these limitations, it is now well understood that removing metadata such as patient name or date of birth is often not enough to preserve privacy. It is, for example, possible to reconstruct a patient’s face from computed tomography (CT) or magnetic resonance imaging (MRI) data. Another reason why data sharing is not systematic in healthcare is that collecting, curating, and maintaining a high-quality data set takes considerable time, effort, and expense. Consequently such data sets may have significant business value, making it less likely that they will be freely shared. Instead, data collectors often retain fine-grained control over the data that they have gathered. Thus decentralized approach to train models provides privacy, security, regulatory and economic benefits. Because federated learning protects privacy, it has attracted a lot of interest. These days, a lot of commercial projects are aiming to develop and use this technology because of its bright future.

Traditional federated learning, however, faces convergence performance issues due to the Non-i.i.d. nature of client data[1]. Several research works have demonstrated that when there is significant client variety, the FedAvg algorithm loses accuracy [2]. The system can experience decreases of up to 51.31 percentage in test accuracy and performance in cases with highly skewed data distributions [3]. In particular, non-i.i.d. data can significantly increase this divergence because of the increased variation in the data distribution, whereas IID data across clients maintains low divergence in weights for each client [3]. Furthermore, the resources of client devices—such as sensors and mobile phones—are usually limited, which reduces their ability to do local training [4]. These training procedures use millions of deep learning algorithms. (FedSiKD: Clients Similarity and Knowledge Distillation: Addressing Non-i.i.d. and Constraints in Federated Learning)

Heterogeneity refers to diversity, systems that use more than one kind of processors or cores (this is known as Heterogeneous Computing) to achieve optimal performance and energy efficiency. In the context of Machine Learning and FL, Heterogeneity concerns data, privacy, and task requirements. Due to different hardware and network connections, the computing and communication capabilities of each device in the federated network may be different. Devices which are simultaneously active in a network usually account for only a small portion. For example, a millions of devices network sometimes only has hundreds of active devices simultaneously. Each device may also be unreliable, thus the heterogeneity of these systems greatly exacerbates the challenges of fault tolerance. Therefore, federated learning methods must tolerate heterogeneous hardware and be robust to offline devices in the network.

So, to conclude  FL enables collaborative model training on data silos in a privacy-preserving manner, which sets it apart from the CML setting. In addition, FL is communication-efficient as it only transfers model parameters which are a fraction in size compared to transferring raw data.

\textbf{ ALSO WRITE HOW ALGO WORKS ON NON IID DATASETS.}

\textbf{Didnt find useful}

In the federal setting, the flexibility of local updates and customer participation affect the training validity of the overall model. In [50], a model called FedProx is proposed, which combines edge device data for distributed training, and uses a federal average [18] model optimization method to ensure the robustness and stability of the target task. Federated Averaging (FedAvg) [18] is the most common model optimization method in federated learning. This method averages the randomly declining gradient data uploaded locally, and then updates it and distributes it back locally (A survey on federated learning). FL could be extended to bring cross-organizational enterprise into federal framework. For instance, bank that possess data of clients’ purchasing power could cooperate with electronic business platform which possess data of product features, to recommend products. Thus, intelligently construct joint model for multiple entities, multiple data sources, different feature dimensions. This enable all to realize cross-platform and regional cocreation value on the premise of protecting data privacy. 

\section{K-Means Clustering}
Clustering is one of the fundamental tasks in data analysis and signal processing, and plays an important role in various applications such as social network analysis, image and video processing and autonomous driving. The unsupervised classification of data elements into groups is known as clustering. K-Means algorithm is an unsupervised clustering algorithm that uses distance measure to separate data points into clusters. Euclidean distance is used to calculate the measure between centroids and each data point. Distributed clustering algorithms are becoming increasingly crucial as independent data sources rise. Clustering data using K-means is a common technique.

\section{Future}
Studying multi-center federated learning to solve
heterogeneous challenges is a promising direction in future work.
Malicious Attacks - Whereas security
attacks can be mostly induced by the presence of malicious clients
in the learning, and they can be either targeted or non-targeted.
In targeted attacks, the adversary wants to manipulate the labels
on specific tasks. Whereas in non-targeted attacks, the motivation
of the adversary is just to compromise the accuracy of the global
model. The defense mechanisms require to detect malicious devices
and remove them from further learning or nullify the effect on the
global model induced by the malicious devices. 
Model Poisoning attacks are similar to data poisoning attacks,
where the adversary tries to poison the local models instead of
the local data. The major motivation behind the model poisoning
attack is to introduce errors in the global model. The adversary
launches a model poisoning attack by compromising some of the devices and modifying it’s local model parameters so that the accuracy
of the global model is affected.
Secure averaging in federated learning lets the devices to be anonymous during the model updating process. Using the same functionality, a device or a group of devices can introduce a backdoor
functionality in the global model of federated learning [3]. Using a
backdoor, an adversary can mislabel certain tasks without affecting
the accuracy of the global model. For instance, an attacker can
choose a specific label for a data instance with specific characteristics. Backdoor attacks are also known as targeted attacks. The
Intensity of such attacks depends on the proportion of the compromised devices present and model capacity of federated learning
[31] .
(Federated Learning: Opportunities and Challenges)
FL with block-chain technology
\\
Because of the decentralized nature of FL, however, it is
susceptible to poisoning attacks [4] if one or more clients intends to sabotage the global model. A poisoning attack is generally categorized into one of two types: untargeted, where
the goal of the adversary is to bring the accuracy of the model
down, or targeted, aiming to bring the accuracy down for a
specific predetermined input. In order to achieve this an adversary can launch a poisoning attack either by manipulating
the available data (data poisoning attack) or by uploading malicious gradients for the model it has trained (model poisoning
attack). In order to mitigate the effect of an attack launched
by malicious clients there have been several robust aggregation algorithms devised to combat this issue in a single-server
configuration
\\
Depending on the capabilities of the adversary, there are
two main ways of performing those attacks - either through model poisoning or data poisoning. Data poisoning occurs
when the training data available on a compromised client to
skew it towards the desired result. The other way is through
model poisoning, where the weights of the model are adjusted
either during or after training with the goal of manipulating
the global model when taken into aggregation.

\section{Personalized FL}

For example, given “I live in the state of”, ideally, it should guess the state the user intended to type. However, suppose we train a single model on all the user data and deploy it, then the model would predict the same state for all users and would not be a good model for most. Similarly, in many practical applications, the distribution of data across clients is highly non-i.i.d. and training a single global model for all clients may not be optimal. Thus, we study the problem of learning personalized models, where the goal is to train a model for each client, based on the client’s own dataset and the datasets of other clients.

However, the general FL approach faces several fundamental challenges: 1) poor convergence on highly heterogeneous data and 2) lack of solution personalization. These issues deteriorate the performance of the global FL model on individual clients in the presence of heterogeneous local data distributions and may even disincentivize affected clients from joining the FL process. Compared with traditional FL, PFL research seeks to address these two challenges. In FL, when the statistical diversity increases(i.e. non-IID data), generalization errors of the global model on clients’ local data also increase significantly. On the other hand, individual learning without FL (i.e., no client collaboration) will also have large generalization error due to insufficient data. These raise the question: How can we leverage the global model in FL to find a
“personalized model” that is stylized for each client’s data?
The key challenge in PFL is to benefit from joint training while allowing each client to keep its own unique model and at the same time limit the communication cost.  


We consider the following three categories of pFL methods
that focus on aggregating models on the server: (1) Methods that learn a single global model and fnetune it.(2) Methods that learn additional personalized models.(3) Methods that learn local models with personalized (local) aggregation.
Many different approaches to PFL have been proposed,
such as: user clustering and collaborating, transfer
learning, multi-task learning, and meta-learning.
One emerging approach to PFL is the use of hypernetworks
instead of a standard federated learning architecture.
Recently, Li et al(the ditto paper) suggested
that personalization can be leveraged not only to improve accuracy, but also to allow for competing
constraints such as robustness and fairness. 
These methods learn
a personalized model by extending meta-learning, local
fine-tuning, multi-task learning, model regularization, contextualization, and model interpolation
Our evaluation results show that the personalized
model with the highest average accuracy across users need
not necessarily be the fairest.
Despite PFL allowing clients to have more control over
their local models, the concept of demographic group fairness,
especially the idea of fairness heterogeneity, in PFL has not
been explored.
\\
 Lastly, these
works employ different data-split strategies among users. these issues make it difficult for a uniform comparison of the effectiveness of each method.(but in our case we had compared different methods/algos on same dataset with same data-split strategies for all.)
\\
Even very simple variants of FedAvg,
such as LGD, which should be easier to analyze, fail to provide theoretical improvements in
communication complexity over their non-local cousins, in this case, GD (Khaled et al., 2019, 2020).1
This observation is at odds with the practical success of local methods in FL. This leads us to
ask the question:
If LGD does not theoretically improve upon GD as a solver for the traditional global
problem (1), perhaps LGD should not be seen as a method for solving (1) at all. In such
a case, what problem does LGD solve?
A good answer to this question would shed light on the workings of LGD, and by analogy, on the
role local steps play in more elaborate FL methods such as local SGD (Stich, 2020; Khaled et al.,
2020) and FedAvg
\\
Another way of personalization is to use Knowledge Distillation (KD) in heterogeneous FL systems.
The principle is to aggregate local soft-predictions instead of local model parameters in the server,
whereby each client can update the local model to approach the averaged global predictions.
Knowledge distillation and personalized federated learning functioned effectively to overcome a
number of federated learning issues, such as data heterogeneity
\\
\section{Unsupervised FL}
Actually, in most of cases where labeled data either do not exist, or
with little existence, unsupervised learning methods are supposed to be
applied. Thus, unsupervised learning is reasonable to be used to infer
potential information in these messy data.
\\
Federated learning is generally used in tasks
where labels are readily available (e.g., next word
prediction). Relaxing this constraint requires design of unsupervised learning techniques that can
support desirable properties for federated training: robustness to statistical/systems heterogeneity, scalability with number of participants, and
communication efficiency. 
\\
Federated Learning (FL) (McMahan et al., 2017) enables
collaborative training of machine learning models while
avoiding transfer of raw data from clients to server. As
remarked by Li et al. (2019), recent work on this topic focuses on addressing the issues of statistical and systems
heterogeneity (Li et al., 2020a; Karimireddy et al., 2020;
Hsu et al., 2019; Zhao et al., 2018; Hsieh et al., 2020);
achieving scalability, privacy, and fairness for participating clients (Charles et al., 2021; Bonawitz et al., 2017; Li et al.,
2020b; 2021b; Smith et al., 2017); and improving communication efficiency (Acar et al., 2021; Konecnˇ y et al. ´ , 2016;
Reddi et al., 2021; Lai et al., 2021). However, existing FL algorithms generally assume a participating client holds high
quality labels that can be used for gradient-based local training (McMahan et al., 2017).
\\
This work considers unsupervised learning
tasks being implemented within the federated learning
framework.the accuracy of federated
learning training reduces significantly when the data is
nonuniformly distributed across devices. 
\\
Federated learning solves
data volume and privacy issues by leaving user data on devices, but
is limited to use cases where labeled data can be generated from
user interaction. Unsupervised representation learning reduces
the amount of labeled data required for model training
\\
It is often the case in practice that unsupervised learning is used as part of a machine learning pipeline (for
instance, to perform dimensionality reduction or representation
learning via SVD) or as a standalone model (for example, to derive
a customer segmentation via k-means). It is thus crucial to develop
approaches towards fair unsupervised learning.
\\
Unsupervised learning (as well as semi-supervised and self-supervised learning) has recently been considered one of the next great frontiers for AI [8]. Unlabeled data far surpasses labeled data in real-world applications. Hence its integration with federated contexts is mandatory to fully unleash the potential of this approach.
In this paper, we consider nodes that have to learn a common ML model (e.g., a classifier). We assume that sets of these nodes “see” similar data patterns. However, as we assume that data are not labeled, nodes need to automatically group themselves into those sets, to perform FL across members of the same set. 
Very few works combining federated learning and unsuper-vised approaches have been released, each of them dealing with limited scenarios and settings. Reference [18] is the first to introduce unsupervised representation learning in a federated setting, but it simply combines the two concepts without assuming the typical issues of distributed settings,
Reference [19] make progress on the same problem by adding and facing two relevant challenges: (i) inconsistency of representation spaces, due to non-IID data assumption, i.e., clients generate local models focused on different categories; (ii) misalignment of representations, given by the absence of unified information among clients.

Reference [20] introduced an unsupervised federated learning (FL) approach for speech enhancement and separation with non-IID data across multiple clients. An interesting aspect of this work is that a small portion of supervised data is exploited to boost the main unsupervised task through a combination of updates from clients, with supervised and unsupervised data.

In [21] authors present a first effort for introducing a collaborative system of autoencoders for distributed anomaly detection. However, the data collected by the edge devices are used to train the models in the cloud, which violates an essential FL feature. Locally, the models are used for inference only.

A more recent work [22] in a similar direction proposes a federated learning (FL)-based anomaly detection approach for identification and classification intrusion in IoT networks using decentralized on-device data. Here the authors use federated training rounds on Gated Recurrent Units (GRUs) models and keep the data intact on local IoT devices by sharing only the learned weights with the central server of the FL. However, dealing with a classification task still assumes the availability of labeled data.
(Anomaly Detection Through Unsupervised Federated Learning)
\\
In [16], unsupervised FL is considered for the case where client data is subdivided into unlabeled sets treated as surrogate labels for training. The authors in [17] exploited similarities across locally trained model embeddings to correct the local models' biases.(Embedding Alignment for Unsupervised Federated Learning via Smart Data Exchange)
\section{Fairness in Unsupervised FL}
More broadly, recent advances have been made recently in the
space of fair unsupervised learning, in particular by introducing
fairlets [9], leading to fair PCA [36, 37], fair k-medoids [3, 17, 25]
and fair spectral clustering [27]. Since fairness in this context is not
obvious to tackle, there have been multiple attempts to define it.
A recent overview of fair clustering has been given in [8]. On the
other hand, in supervised learning, multiple technical definitions
of fairness co-exist and have been reviewed in-depth [4, 23, 32, 40],
bringing to the fore impossibility theorems [10, 24] that proved that
these different acceptations of fairness cannot be satisfied at once.
In addition, it has been shown that [2, 23, 34] fully debiased models
could fail to generalise out-of-sample, which we would expect to
also apply to the case of unsupervised learning. The relationship between fairness in supervised and unsupervised
learning is not straightforward. Many notions of fairness in supervised learning (such as classification and scoring [11, 19, 24]) focus
on a single learning task, whereas unsupervised learning considers
a generic transformation of the data. While fairness in unsupervised
learning has recently become a major theme of research, fair PCA
–for instance– can be seen directly in the line of earlier attempts to
reduce the correlation between a protected (or sensitive) attribute
[6, 41].
For the sake of brevity, we do not give an exhaustive account of
fairness in unsupervised learning. It is tempting to consider [31] as
an early attempt at introducing (invidual) fairness in clustering. By
adapting the notion of disparate impact to clustering and introducing the notion of fairlets (i.e., minimal sets that satisfy fair representation while approximately preserving the clustering objective), [9]
paved the way for much of the work in the field. [36, 37] explore
PCA and dimensionality reduction with multiple constraints, with
an application to fairness. In [27], the authors tackle the case of
spectral clustering. [1] proposes a generic approach to fair clustering, including k-medoids and considers a minmax criterion across
groups. On a different note, [7] tackles the issue of data summarisation via a determinantal measure of diversity. Furthermore, work in fair recommender systems (which include
some matrix factorisation techniques) has grown due to the better understanding of certain phenomena such as echo chambers
or filter bubbles. In addition to biases linked to certain protected
characteristics (such as poor performance of recommender systems
to serve under-represented minority groups), specific issues have
appeared such as user under-representation [29] and item underrecommendation (also known as popularity bias) [42].
As a result of unsupervised learning’s diversity and breadth, multiple notions of fairness have been put forward for (or adapted to)
unsupervised learning, including social fairness, balance fairness
and individual fairness. Let us now give a brief account of these
different criteria.

(1) The social fairness criterion was introduced in unsupervised
learning in [17], where it was applied to a clustering problem
and further developed in [1, 30]. In short, it requires that the
average cost (e.g., reconstruction loss in PCA or distance to
medoid in clustering) be the same across groups. This can be
tackled by minimising the maximum of groups’ average costs.

(2)Similarly, the principle according to which different groups
should have the same distribution across clusters can be
traced back to [9], where the authors posit the notion of balance fairness, which they attack through so-called “fairlets”.
A related concept is that of bounded representation [3], which
requires that the proportion of a group in each cluster be
between two pre-specified values. The maximum fairness
cost [17] is the maximum of the sum of all deviations from
the ideal proportion for each protected group in a cluster.

(3) Last, individual fairness compares the statistical distance
between two points obtained from their inputs and the algorithm’s output distribution and mandates that two similar
inputs should have similar outputs. This paradigm was first
used in [31] for clustering and further adapted by [26].

(Towards Fair Unsupervised Learning....refer for fairness its nice fairness history wise amd types)


==> related_work.tex <==
\section{Related Work}
----------------------------------------------------------
Federated Clustering
-----------------------------------------------------------
(a) https://arxiv.org/abs/2210.16524  (Tarushi)
(b) https://docs.google.com/viewer?url=https%3A%2F%2Ffederated-learning.org%2Ffl-aaai-2022%2FPapers%2FFL-AAAI-22_paper_48.pdf&pdf=true --> Generative   ,,,,,,,,,,,,
(c) https://www.sciencedirect.com/science/article/abs/pii/S1574119222001390 --> In SS-FedCLAR , each client uses a combination of active learning and label propagation to provide pseudo labels to a large amount of unlabeled data, which is then used to collaboratively train a Federated Clustering model.
(Tsering)

(d) https://arxiv.org/abs/2310.15330 --> federated gradient EM algorithm (FedGrEM) designed for the unsupervised learning of mixture models, which supplements the existing federated EM algorithms by considering task heterogeneity and potential adversarial attacks. 


(e) https://ieeexplore.ieee.org/abstract/document/9516933-->(Tsering)

(f) https://ieeexplore.ieee.org/abstract/document/9693930 --> application of federated clustering to electircity pattern (Tsering)

(g) https://docs.google.com/viewer?url=https%3A%2F%2Fpure.tue.nl%2Fws%2Fportalfiles%2Fportal%2F278830245%2FLeeuw_W.pdf&pdf=true  --> Need to read (This research presents a novel process to train clustering models collaboratively without compromising accuracy while accommodating privacy and security in a decentralized manner. To decentralize collaborative learning and remove the single point of failure, a consensus is instead built collaboratively to facilitate the federated learning task. We present a committee-based consensus method designed for blockchain-based federated learning that is more scalable than common

(h) https://link.springer.com/article/10.1007/s10115-024-02066-x--> Read


(i) https://arxiv.org/abs/2201.07316 --> shyd upar ka hi arixv h checlk  (Tarushi)

(j) https://arxiv.org/abs/2205.15564 --> Secure FC --> old papers have line   ,,,,,

(k) https://www.mdpi.com/2076-3417/12/20/10455  --> Important Read --> In this paper, we introduce a federated clustering framework that solves three challenges: determine the number of global clusters in a federated dataset, obtain a partition of the data via a federated fuzzy c-means algorithm, and validate the clustering through a federated fuzzy Davies–Bouldin index (Tsering)

(l) https://link.springer.com/chapter/10.1007/978-3-031-27609-5_3  --> (READ) that allows to learn clusters from distributed homogeneous data without sharing it. method is its ability to retain, merge and discard original clusters sent by data owners. (Tarushi) (no access till now) (mailed now copy pdf from authors)


(m) https://arxiv.org/abs/2305.01068  --> FedGMM, which utilizes Gaussian mixture models (GMM) to effectively fit the input data distributions across diverse clients. The model parameters are estimated by maximum likelihood estimation utilizing a federated Expectation-Maximization algorithm, (Tarushi) (should see again)

https://arxiv.org/pdf/2402.12852.pdf
https://www.ncbi.nlm.nih.gov/pmc/articles/PMC10898505/
https://www.techrxiv.org/doi/full/10.36227/techrxiv.170258792.25216957 - One-shot Federated K-means Clustering based on Density Cores  (Very similar to our paper :( :( ) crying in corner !!  ek difference h ke hum personalization krrhe todhi but main algo theme same h... which reduces slightly novelty... but abhi yeh unpublished h sirf arxiv p h but close h toh woh dikat... let me see more closely to it. 

Privacy-preserving federated deep clustering based on gan

k-PFED: Communication-efficient Personalized
Federated Clustering (bekar paper non understandable) 
------------------------------------------ -----------------------------
Federated Unsupervised Learning (FedUL)
-----------------------------------------------------------------------

(a) https://ieeexplore.ieee.org/abstract/document/9632783 --> speech enhancement and separation with non-IID distributed data across multiple clients. We simulate a realworld scenario where each client only has access to a few noisy recordings from a limited and disjoint number of speakers (hence non-IID).

(b) https://www.sciencedirect.com/science/article/abs/pii/S0167404823000160 --> Intrusion Detection 

(c)  https://docs.google.com/viewer?url=https%3A%2F%2Farxiv.org%2Fpdf%2F2002.11545.pdf&pdf=true  --> Survey 

(d) https://arxiv.org/abs/2308.05870 --> investigates FL paradigm in a resource-constrained and label-missing environment. Specifically, we propose a novel framework of UFed-GAN: Unsupervised Federated Generative Adversarial Network, which can capture user-side data distribution without local classification training.



                   -------------------------------
                    Client Clustering 
                   -------------------------------

(a) https://arxiv.org/abs/2205.11506 -->  a novel unsupervised federated learning technique that exploits the federation's hierarchy to orchestrate a distributed clustering task and enforce a globally consistent partitioning of clients' data into discriminable clusters.

(b) https://ieeexplore.ieee.org/abstract/document/10076669-->  aim to extend the FL paradigm to unsupervised tasks by addressing the problem of anomaly detection (AD) in decentralized settings. In particular, we propose a novel method in which, through a preprocessing phase, clients are grouped into communities, each having similar majority (i.e., inlier) patterns. Subsequently, each community of clients trains the same anomaly detection model (i.e., autoencoders) in a federated fashion. The resulting model is then shared and used to detect anomalies within the clients of the same communi

(c) https://link.springer.com/chapter/10.1007/978-981-16-4963-9_6  --> Dual Averaging (DA), where the gradients of each agent are aggregated at a central node.//
two weight computation algorithms, with one using a fixed size bin and the other with self-organizing maps (SOM) that solves the underlying dimensionality problem inherent in the first me
 Unsuper FEDL

 
(d) https://arxiv.org/html/2403.04144v1




---------------------------------------------------------
Federated SemiSupervised Learning (FedSSL)
---------------------------------------------------

(a) https://www.mdpi.com/2227-7390/11/8/1972 -> server node can provide (i) a pre-trained model to help each client node annotate the local data uniformly and (ii) an estimation of the global gradient to help correct the local gradient.

(b) https://www.sciencedirect.com/science/article/abs/pii/S1574119222001390 --> In SS-FedCLAR , each client uses a combination of active learning and label propagation to provide pseudo labels to a large amount of unlabeled data, which is then used to collaboratively train a Federated Clustering model.

(c) https://odr.chalmers.se/items/f84f18e6-61b8-4df3-a3c6-44564bb8c5ce --> thesis for auto driving semi techni for unlabelled data

(d) https://www.sciencedirect.com/science/article/abs/pii/S1568494623004714

(e) https://docs.google.com/viewer?url=https%3A%2F%2Farxiv.org%2Fpdf%2F2303.14453.pdf&pdf=true --> Survey unlabelled 

(f) https://arxiv.org/abs/2108.09412

(g) https://arxiv.org/abs/2110.02470


---------------------------------------------------------------
Federated Unsupervised Representation learning  (FedURL)
-------------------------------------------
(a) https://dl.acm.org/doi/abs/10.1145/3378679.3394530 --> Unsupervised representation learning reduces the amount of labeled data required for model training, // learning to pre-train deep neural networks using unlabeled data in a federated setting. Pre-trained networks can be used to extract discriminative features. The features help learn a down-stream task of interest with a reduced amount of labeled data.

(b) https://link.springer.com/article/10.1631/FITEE.2200268

(c) https://link.springer.com/chapter/10.1007/978-3-031-20056-4_40 --> Our model learns unbiased representation from decentralized and heterogeneous local data. It employs a two-sided knowledge distillation with contrastive learning as a core component, all


---------------------
Left out (Pdf check)
-----------------------

(a) https://ieeexplore.ieee.org/abstract/document/9348203 (Federated Clustering for Electricity Consumptio) 
(b) https://openaccess.thecvf.com/content/ICCV2023/html/Kim_ProtoFL_Unsupervised_Federated_Learning_via_Prototypical_Distillation_ICCV_2023_paper.html

(c) https://ieeexplore.ieee.org/abstract/document/9693930


---------------------------
COmpletely different but cite as words in title
---------------------------
(a) https://dl.acm.org/doi/abs/10.1145/3476883.3520221--> discarding the weights update of clients, we propose a novel robust federated learning method that utilizes Metrics Learning to encode the local data and leverages the unsupervised clustering method K-means to preclude malicious data during local training.


(b) https://arxiv.org/abs/2307.15994-- > cite  in personalization  (federated model has been trained and deployed, and an unlabeled new client joins, providing a personalized model for the new client becomes a highly challenging task)

(c) https://link.springer.com/chapter/10.1007/978-981-19-2397-5_3 --> Wherein, the first phase of the algorithm divides the data into different sub-clusters based on the density evaluation with respect to all the data dimensions and, in the second phase, the small sub-clusters are federated with large sub-clusters to create the actual data clusters.



-------------------------
Fairness in Fed 
-----------------------
(a)https://ieeexplore.ieee.org/abstract/document/10008103  --> Read paper

------------------------------
See later if cite
-----------------------

(a) https://arxiv.org/abs/2102.10799--> In this paper, we have proposed an approach that detects the adversaries with the help of a clustering algorithm. After clustering, it further rewards the clients for detecting honest and malicious clients


(b) https://arxiv.org/abs/2210.16424 --> Machine unlearning of Federated clusters 

(c) https://arxiv.org/abs/2302.11823

(d) Unsupervised clustering of MDS data using federated learning


----------------------
APplication papers
-------------------

(a) https://link.springer.com/chapter/10.1007/978-3-030-23551-2_2 --> Credit Card Federated learing 








----------------------
Extra
--------------------

(a) https://link.springer.com/chapter/10.1007/978-981-99-9637-7_28
(b) https://openreview.net/forum?id=djwnKXz1B2
(c) https://docs.google.com/viewer?url=https%3A%2F%2Ffindresearcher.sdu.dk%2Fws%2Fportalfiles%2Fportal%2F202008017%2Fmain.pdf&pdf=true


==> related_work2.tex <==
\section{Related Work}
%%%Machine learning (ML) encompasses various paradigms, including supervised learning with labeled data and unsupervised learning for discovering patterns in unlabeled data. Traditional ML often requires centralized access to data, which may raise privacy concerns when dealing with sensitive information.

%%%Federated Learning, an emerging paradigm, addresses these challenges by enabling collaborative model training across decentralized devices or entities without sharing raw data. There is a significant body of literature focused on supervised federated learning [\cite{fedssc}, \cite{fedmix}, \cite{federatedTraffic}, \cite{secureFL}, \cite{decentralizedFL}, \cite{federatedTL}, \cite{lobner2022enhancing}, \cite{banerjee2020multi}, \cite{saputra2019energy}, \cite{hsu2020federated}].Research into unsupervised learning (UL) is still in its early phases [\cite{chung2022federated}, \cite{kFED}] but gaining traction, especially given the growing availability of unlabeled data.In unsupervised settings, federated learning extends to federated clustering, where multiple parties collaborate to discover patterns and structures in distributed datasets while preserving data privacy as in \cite{FedEg}.  %Fed Eg new example electricity wala

In this section, we have structured our discussion into two parts. The first segment elucidates the landscape of federated learning, highlighting key research and developments in the field. Following this, the second part delves into the crucial aspect of fairness within federated learning frameworks, examining its challenges and emerging methodologies.

% 2020:
% Fairness and Accuracy in Federated Learning

% 2021: (done)
% (e) Federated FCM: Clustering Under Privacy Requirements(Tsering)(done)
% March: KFED **
% Oct: FairFed**
% Nov: Unified Group Fairness on Federated Learning**

% 2022:
% (i) 18 Jan: Towards Federated Clustering: A Federated Fuzzy c-Means Algorithm (FFCM)(Tsering) (done)
% (f) Jan: Federated Clustering for Electricity Consumption Pattern Extraction(done)
% May: SecFC**
% (g) June: BC-FL k-means: A Consortium Blockchain for Federated Clustering (done)
% (a) 29 Oct: Federated clustering with GAN-based data synthesis (Tsering) (done)
% On a Framework for Federated Cluster Analysis 

% 2023:
% Jan: Federated Clustering and Semi-Supervised learning for sensor-based Human Activity Recognition(HAR). 
% (l) 08 March : FedCLUS: Federated Clustering from Distributed Homogeneous Data (Tsering) (done)
% (m) 1 May: Personalized Federated Learning under Mixture of Distributions (Tsering)(GMM hi h) (done)
% Sept: MFC**
% (d) 23 Oct: Towards the Theory of Unsupervised Federated Learning: Non-asymptotic Analysis of Federated EM Algorithms (Fed EM)
% Greedy centroid initialization for federated K-means(Tsering)(done) **  // isko see and add
% 2024:
%Jan: One-shot Federated K-means Clustering based on Density Cores(Tarushi) (done)
%Jan: CCFC
 
\textbf{Federated Clustering: }

One of the early works in unsupervised federated learning focussed on soft clustering. In \cite{FedFCM} algorithmic framework for federated fuzzy clustering and thus Fuzzy C-Means federated version was developed where for each client their partition matrix was updated whenever each time server sent the updated global centers which in turn were updated using gradient of weighted sum of euclidean distance of datapoints and global centers. In a more advanced version proposed in \cite{ArchiFedFCM} iterative fuzzy c-means algorithm is extended to federated learning where fuzzy c-means algorithm is run multiple times between the server and client till convergence is achieved. However since it is a soft clustering, each data point is assigned probabilities across multiple global centers in federated fuzzy clustering. So no definitive assignment of each data point to a single center is achieved.

% One of the early works done in unsupervised federated learning is by \cite{FedFCM} in which they developed an algorithmic framework for federated fuzzy clustering and Fuzzy C-Means federated version where for each client, there is a partition matrix(define partition matrix) which is updated each time server send the updated global centers. And for updating global centers, each client send the gradient of weighted sum of euclidean distance of datapoints and global centers.

% Moving on, to federated fuzzy c-means algorithm (FFCM) \cite{ArchiFedFCM}. In this paper, iterative fuzzy c-means algorithm is extended to federated learning. Clients locally run number of fuzzy c-means iterations and send the local centers to server. Server then updates the global centers and send them back to the clients who uses them to update their local centers. This process is repeated until convergence. 

% It is crucial to highlight a significant outcome: each data point is initially assigned probabilities across multiple global centers in federated fuzzy clustering. However, an essential objective of our research, as outlined in the literature, is to achieve a definitive assignment of each data point to a single global center. 

The work in federated data clustering is in the formative stages. The initial attempt to explore the partitioning of data points scattered across multiple devices into k clusters is provided in \cite{kFED}. The authors propose an algorithm (k-FED) based on the famous offline Llyod’s heuristic (usually named offline k-means). The algorithm uses the Llyod heuristic locally on each device and then computes the final clustering in only one round of communication. Though it is communication efficient, the performance of k-FED is highly dependent on the data distribution across clients. We further show that k-FED suffers significant fluctuations in the clustering cost across different client devices.

A work in privacy-preserving distributed clustering is achieved using cryptographic techniques while still allowing for accurate clustering in \cite{SedFC} . In this, the clients perform local center updates and share encrypted distance vectors using lagrange encoding back to the server. The server is then responsible for gathering all secret distance codes from the clients and carrying out the following iteration updates. Though the algorithm leverages the beneﬁts of encryption-decryption to protect data privacy, such methods require signiﬁcant computation overhead and communication costs.The sharing of distance vectors can hinder the scalability of the technique.

Considering blockchain's inherent security properties, aiming to leverage its decentralized and immutable nature to address the challenges posed by traditional federated learning, \cite{BCFL}, a blockchain-based approach that employed the federated k-means clustering algorithm within a committee-based consensus protocol was proposed. It performed similar to centralized k-means if data is IID distrobuted. It reach convergence in many cases, even when data is non-IID distributed and the proportion of malicious devices is high. However, The use of blockchain alongside federated learning, came with an increase in runtime compared to traditional federated learning and only marginally helps in alleviating issues in traditional federated learning like regarding privacy.   

% \cite{BCFL} presented a blockchain-based framework for federated learning in which federated k-means clustering algorithm was applied. The framework included a committee-based consensus protocol designed with collaborative learning in mind and a reputation system to improve convergence and global model quality which performs similarly to centralized k-means if data is IID distributed. It reach convergence in many cases, even when data is non-IID distributed and the proportion of malicious devices is high. However, The use of blockchain alongside federated learning, on the other hand, comes with an increase in runtime compared to traditional federated learning and only marginally helps in alleviating issues in traditional federated learning like regarding privacy. 

Another approach, as demonstrated by the work of \cite{GAN}, involves the generation of synthetic data at the server level, aiming to attain global cluster centers without directly utilizing original data.

% A different line of work includes the work by \cite{GAN} that attempts to achieve global cluster centers by generating synthetic data at server instead of using original data.

Yet another work combining benefits of Federated Clustering and Semi-Supervised learning was proposed in \cite{SSFedClar} where clients provide pseudo labels to a large amount of unlabelled data, which is used to train Federated Clustering model. While the reliance on labeled data has reduced however, it does not eliminate this requirement entirely. A small amount of labeled data is still necessary at the outset to initialize the process. 

% \cite{SSFedhe need for labelled dataClar} proposed a novel combination of Federated Clustering and Semi-Supervised learning for sensor-based Human Activity Recognition(HAR). Each client uses a combination of active learning and label propagation to provide pseudo labels to a large amount of unlabeled data, which is then used to collaboratively train a Federated Clustering model. Though in this method the need of labelled data is reduced it is not finished completely i.e. initially small amount of labelled data is still needed.

In certain studies, DBSCAN has been employed for local clustering tasks. For instance, in \cite{FedClus}, a modified DBSCAN algorithm is executed locally by clients to produce local clusters characterized by centroid, size, radius, and density. These local clusters are then sent to the server, which utilizes these cluster properties to compute global centers, subsequently sending them back to the clients. 

% \cite{FedClus} - In this paper, clients locally run a modified DBSCAN (which includes centroid, size, radius and density of the cluster) to generate local clusters. The server receives them and here they took three cases of how the received clusters might be. Case 1, if any 2 clusters are overlapping then the dominant one(w.r.t size, radius and density) is chosen and the other one is discarded. If they just touch each other, then a new cluster is created by taking mid point of the centrioids and half of the sum of their radii. And if they are absolutely distinct clusters, then both of them are considered. These are finally send back to clients as they assign their datapoints to these final clusters. They have not made any assumptions regarding the number of clusters generated by the clients.

One of the latest work done in the federated clustering is by \cite{GreedyCentroid}. In the algorithm firstly clients run kmeans or kmeans++ to generate set of local centers and send these centers along with the number of datapoints assigned to these clusters to the server. At server, they choose the first center among all the shared centers considering the sum distance of all the datapoints.It then follows by choosing next center which is not closer to the already choosen center or the center with relatively less number of datapoints. Then the server sends back the global centers and clients updates their local centers. This is repeated until convergence. However, despite their attention to Non-IID datasets, they have notably neglected experimentation with IID datasets, leaving a gap in understanding the broader applicability of their findings. Moreover, the identified drawbacks encompass not only low efficiency but also the considerable computational costs associated with the implementation.

% One of the latest work done in the federated clustering is by \cite{GreedyCentroid}. Firstly clients runs kmeans or kmeans++ to generate local centers and send them to the server. But along with the local centers. they send an additional information of number of datapoints assigned to that particular center which helps the server to better choose the global center. At server, they choose the first center among all the shared centers which minimizes the sum distance of all the datapoints. This center in a way best represents all the datapoints. It then follows by choosing next center which is not closer to the already choosen center or the center with relatively less number of datapoints. Then the server sends back the global centers and clients updates their local centers. This is repeated until convergence.

Yet another innovative approach was proposed by \cite{CCFC} where they use a cluster contrastive model which is a more general form of simple Siamese networks and focus mainly on clustering images by embedding the cluster-contrastive model into the FedAvg framework. However, it suffered from heterogeneous data across clients, leading to poor and unrobust performance. To mitigate this \cite{CCFC++} was introduced which involved a decorrelation regularizer to diminish the detrimental effects of data heterogeneity, particularly addressing the issue of dimensional collapse of the learned representations.

% Yet another type of method was proposed by \cite{CCFC} where they use a cluster contrastive model which is a more general form of simple Siamese networks and focus on clustering images by embedding the cluster-contrastive model into the FedAvg framework with the model-contrastive regularization term while we are using the attributes of images and bringing up fair clustering in federated environment. However, it suffered from heterogeneous data across clients, leading to poor and unrobust performance. To mitigate this \cite{CCFC++} was introduced which involved a decorrelation regularizer to diminish the detrimental effects of data heterogeneity involves addressing the dimensional collapse of the learned representations.

A new federated k-means clustering framework to balance communication costs and clustering effectiveness was introduced in \cite{DPCBased}. Here initially clients use cluster centers (representative points) genearated by K-means to represent the corresponding clusters. The server then reprocess these uploaded encrypted representative points to obtain better final cluster centers by taking the improved density peaks (density cores) as final centers, and then send them back to the clients. Finally, each client assign local data to the nearest centers.The choice of density cores, as detailed in \cite{DPC} is significant because it allows the total number of clusters to be determined solely by the data itself, eliminating the need to specify the number of clusters beforehand. (drawback - k is not fixed, differ for each client, affect overall cost?)

% In 2023 \cite{DPCBased} proposed a new federated k-means clustering framework to balance communication costs and clustering effectiveness in which initially clients use cluster centers (representative points) genearate by K-means to represent the corresponding clusters. The server then reprocess these uploaded encrypted representative points to obtain better final cluster centers by taking the improved density peaks (density cores) as final centers, and then send them back to the clients. Finally, each client assign local data to the nearest centers. However it might affect the fairness across clients as the overall cost for each client may vary a lot due to the fact that the final density cores are decided upon by \cite{DPC} and their special property is that the total number of clusters depend entirely upon the data i.e. we do not provide the number of clusters to be generated which would end up bringing huge difference in clustering cost across clients.

\textbf{Federated Clustering and Fairness: }

The shift from a centralised to decentralised also introduced a critical challenge: the imperative for fairness in federated learning. With data dispersed across various nodes and devices, ensuring equitable representation and treatment becomes paramount. 
% In this journal, we delve into the complexities of fostering fairness in federated learning, exploring strategies, challenges, and implications for building an algorithm which is fair towards all clients. (add?)

One among the earlier works on fairness includes \cite{FairAccu} which combines a double momentum gradient and a weighting strategy for a supervised environment. The double momentum gradient takes into account the influence of historical gradient information at both client and server sides to improve the convergence of the algorithm. The weighting strategy aggregates the weights according to the training accuracy and the number of participants to create a fairer and more accurate federated learning algorithm which significantly improves the convergence and fairness of federated learning in heterogeneous environments only. (cnfm supervised??)

% \cite{FairAccu} proposed FedFa, which combines a double momentum gradient and a weighting strategy. The double momentum gradient takes into account the influence of historical gradient information at both client and server sides to improve the convergence of the algorithm. The weighting strategy aggregates the weights according to the training accuracy and the number of participants to create a fairer and more accurate federated learning algorithm which significantly improves the convergence and fairness of federated learning in heterogeneous environments only. 

\cite{FairFed} also known as FairFed highlights a new way to make sure everyone gets a fair shake in federated learning. In a federated setting, each piece of data in a client's device belongs to a different group. FairFed focuses on making sure these groups are treated fairly. With FairFed, each client performs local debiasing on its own local dataset. To amplify the local debiasing performance, the clients will evaluate the fairness of the global model on their local datasets in each FL round until convergence and collectively collaborate with the server to adjust its model aggregation weights.

% 4. \cite{FairFed} is a novel algorithm for fairness-aware aggregation to enhance group fairness in federated learning.Each client performs local debiasing on its own local dataset, thus maintaining data decentralization and avoiding the exchange of any explicit information of its local data composition.To amplify the local debiasing performance, the clients will evaluate the fairness of the global model on their local datasets in each FL round until convergence and collectively collaborate with the server to adjust its model aggregation weights.The weights area function of the mismatch between global fairness fairness measurement and local fairness measurement at each client ,favoring clients whose local measures match the global measure. Thus costing high computational time.

Another notion of fairness named group fairness which focussed on achieving client-level, attribute-level and agnostic distribution fairness simultaneously was introduced in \cite{Unified} where they propose a fair federated framework and a corresponding unified group fairness risk which encourages the model to focus on those groups with high risk, so it helps to achieve group fairness. To optimize the proposed risk for unified group fairness, an efficient federated optimization algorithm named FMDA-M based on mirror descent ascent technique and momentum acceleration with convergence guarantee is proposed. (high level terms?)

% \cite{Unified} investigate a new problem of unified group fairness on FL for achieving client-level, attribute-level and agnostic distribution fairness simultaneously. Theoretically, they propose a fair federated framework and a corresponding unified group fairness risk which encourages the model to focus on those groups with high risk, so it helps to achieve group fairness. To optimize the proposed risk for unified group fairness, an efficient federated optimization algorithm named FMDA-M based on mirror descent ascent technique and momentum acceleration with convergence guarantee is proposed. 

Combining the principles of soft clustering with a focus on fairness led to the development of the framework proposed by \cite{FrameFedClusAnaly}. This innovative federated clustering approach addresses three key challenges within a federated dataset: determining the optimal number of global clusters, achieving data partitioning using a federated fuzzy c-means algorithm, and validating the resulting clusters. The validation measures how well “cluster spread” is balanced against “dissimilarity between cluster centers”. Federated Fuzzy c-Means at client side with k-Means Averaging at server side is used mainly until convergence thus costing high in terms of communication while still being a soft clustering. (fairness ki taraf na??)(cnfm this!!)

% \cite{FrameFedClusAnaly} introduced a federated clustering framework that solves three challenges: determine the number of global clusters in a federated dataset, obtain a partition of the data via a federated fuzzy c-means algorithm, and validate the clustering. The validation measures how well “cluster spread” is balanced against “dissimilarity between cluster centers”. Federated Fuzzy c-Means at client side with k-Means Averaging at server side is used mainly until convergence thus costing high in terms of communication and still being a soft clustering. (fairness ki taraf na??)

Another new approach in federated learning is by implementing personalization in it. A recent example is \cite{GMMBased} which uses a personalised federated learning approach to utilize Gaussian mixture models (GMM) to effectively fit the input data distributions across diverse clients. The algorithm starts by the server broadcasting the aggregated base models to all clients, including Gaussian parameters and supervised learning models. Each client then locally updates the parameter of the base models and the mixture weights and then send the updated components back to the server. The server aggregates the updates. 

% \cite{GMMBased} is a personalised federated learning approach that utilizes Gaussian mixture models (GMM) to effectively fit the input data distributions across diverse clients. The model parameters are estimated by maximum likelihood estimation utilizing a federated Expectation-Maximization algorithm. The algorithm is: server broadcast the aggregated base models to all clients, including Gaussian parameters and supervised learning models. Each client locally updates the parameter of the base models and the mixture weights and then send the updated components back to the server. The server aggregates the updates. 

\cite{MFC} also called Multishot Federated Clustering (MFC) was proposed, which performs well in both heterogeneous and non-heterogeneous settings and utilizes multiple rounds of interaction to achieve much better cost. It not only minimizes the overall clustering cost but also promotes cost fairness across devices. By sending the maximum-cost cluster center from each device to the server, even if a device initially suffers high cost, it will soon reduce and become more equitable with other devices. To assess the effectiveness and fairness achievable with our proposed method, we conducted comparative analyses against MFC,aiming to evaluate and benchmark the levels of fairness attainable in federated clustering scenarios.

% To tackle these issues, \cite{MFC} also called Multishot Federated Clustering (MFC) was proposed, which performs well in both heterogeneous and non-heterogeneous settings and utilizes multiple rounds of interaction to achieve much better cost.It not only minimizes the overall clustering cost but also promotes cost fairness across devices. By sending the maximum-cost cluster center from each device to the server, even if a device initially suffers high cost, it will soon reduce and become more equitable with other devices.

Others - \cite{GanSimi}[\url{https://www.ncbi.nlm.nih.gov/pmc/articles/PMC10898505/}]
\cite{kPFED}[\url{https://ieeexplore.ieee.org/abstract/document/10176651}]
\cite{PrivacyAndFair}[\url{https://dl.acm.org/doi/abs/10.1145/3314183.3323847}]

\cite{FedGrEM} provides a non-asymptotic theory underlying the federated EM algorithms, accounting for task heterogeneity and adversarial contaminations. It seeks to illustrate when and how federated learning can improve local performance and offers novel insights into unsupervised federated learning. However it has an indirect implications on ethical considerations in data handling and algorithm deployment. (smjh ni aara tha)

